The FluidFlower International Benchmark Study: Process, Modeling Results, and Comparison to Experimental Data

Successful deployment of geological carbon storage (GCS) requires an extensive use of reservoir simulators for screening, ranking and optimization of storage sites. However, the time scales of GCS are such that no sufficient long-term data is available yet to validate the simulators against. As a consequence, there is currently no solid basis for assessing the quality with which the dynamics of large-scale GCS operations can be forecasted. To meet this knowledge gap, we have conducted a major GCS validation benchmark study. To achieve reasonable time scales, a laboratory-size geological storage formation was constructed (the "FluidFlower"), forming the basis for both the experimental and computational work. A validation experiment consisting of repeated GCS operations was conducted in the FluidFlower, providing what we define as the true physical dynamics for this system. Nine different research groups from around the world provided forecasts, both individually and collaboratively, based on a detailed physical and petrophysical characterization of the FluidFlower sands. The major contribution of this paper is a report and discussion of the results of the validation benchmark study, complemented by a description of the benchmarking process and the participating computational models. The forecasts from the participating groups are compared to each other and to the experimental data by means of various indicative qualitative and quantitative measures. By this, we provide a detailed assessment of the capabilities of reservoir simulators and their users to capture both the injection and post-injection dynamics of the GCS operations.

==> distances/distances_120h.tex <==
distances, Austin, CSIRO, DARSim, DARTS, LANL, Melbourne, Stanford, Stuttgart
Austin,0.000000000000000000e+00,1.254325625996619842e-01,1.250735221082655002e-01,1.239394475444362959e-01,5.912014317730726054e-01,1.032438464219911783e-01,3.045653570946619260e-01,2.001401833056833113e-01
CSIRO,1.254325625996619842e-01,0.000000000000000000e+00,1.685453787323973884e-01,8.206390504277225051e-02,6.266199849683484757e-01,7.592444235125983543e-02,3.273542557362377758e-01,2.352746253766519469e-01
DARSim,1.250735221082655002e-01,1.685453787323973884e-01,0.000000000000000000e+00,1.567624794999229743e-01,4.851832780615021878e-01,1.298636603084167007e-01,3.694528240306946820e-01,1.386887785487820046e-01
DARTS,1.239394475444362959e-01,8.206390504277225051e-02,1.567624794999229743e-01,0.000000000000000000e+00,5.565570044257037718e-01,7.536834082729698681e-02,3.358872113520132152e-01,1.655297963549857698e-01
LANL,5.912014317730726054e-01,6.266199849683484757e-01,4.851832780615021878e-01,5.565570044257037718e-01,0.000000000000000000e+00,6.033476673088520315e-01,8.538397552364889176e-01,3.922643626146811724e-01
Melbourne,1.032438464219911783e-01,7.592444235125983543e-02,1.298636603084167007e-01,7.536834082729698681e-02,6.033476673088520315e-01,0.000000000000000000e+00,2.712482567823156776e-01,2.140530323070907182e-01
Stanford,3.045653570946619260e-01,3.273542557362377758e-01,3.694528240306946820e-01,3.358872113520132152e-01,8.538397552364889176e-01,2.712482567823156776e-01,0.000000000000000000e+00,4.635872997065152989e-01
Stuttgart,2.001401833056833113e-01,2.352746253766519469e-01,1.386887785487820046e-01,1.655297963549857698e-01,3.922643626146811724e-01,2.140530323070907182e-01,4.635872997065152989e-01,0.000000000000000000e+00


==> distances/distances_24h.tex <==
distances, Austin, CSIRO, DARSim, DARTS, LANL, Melbourne, Stanford, Stuttgart
Austin,0.000000000000000000e+00,1.971440280858478833e-01,2.251655672897716065e-01,1.394451841052679331e-01,7.119447336139315130e-01,2.503947483682851805e-01,3.190875084684624552e-01,1.865564564516187795e-01
CSIRO,1.971440280858478833e-01,0.000000000000000000e+00,7.618612866538880535e-02,1.007941156418644818e-01,5.268500034531935494e-01,1.177699213218299512e-01,4.934463467839097506e-01,3.713102006924403481e-02
DARSim,2.251655672897716065e-01,7.618612866538880535e-02,0.000000000000000000e+00,1.524357537148444686e-01,5.003267096099182076e-01,1.129347225434782498e-01,5.229464217837344053e-01,8.813092250298490415e-02
DARTS,1.394451841052679331e-01,1.007941156418644818e-01,1.524357537148444686e-01,0.000000000000000000e+00,5.909759179659822559e-01,1.403288886012895309e-01,4.284622250438068214e-01,1.178549972347203156e-01
LANL,7.119447336139315130e-01,5.268500034531935494e-01,5.003267096099182076e-01,5.909759179659822559e-01,0.000000000000000000e+00,4.847115950808733031e-01,1.015172760816997366e+00,5.328935269196652946e-01
Melbourne,2.503947483682851805e-01,1.177699213218299512e-01,1.129347225434782498e-01,1.403288886012895309e-01,4.847115950808733031e-01,0.000000000000000000e+00,5.345631346728777489e-01,1.508780944219428322e-01
Stanford,3.190875084684624552e-01,4.934463467839097506e-01,5.229464217837344053e-01,4.284622250438068214e-01,1.015172760816997366e+00,5.345631346728777489e-01,0.000000000000000000e+00,4.896863523495065817e-01
Stuttgart,1.865564564516187795e-01,3.713102006924403481e-02,8.813092250298490415e-02,1.178549972347203156e-01,5.328935269196652946e-01,1.508780944219428322e-01,4.896863523495065817e-01,0.000000000000000000e+00


==> distances/distances_48h.tex <==
distances, Austin, CSIRO, DARSim, DARTS, LANL, Melbourne, Stanford, Stuttgart
Austin,0.000000000000000000e+00,1.579724395270813153e-01,1.940029980493869766e-01,1.460833131822168451e-01,6.468212986499282113e-01,2.016112504502489133e-01,3.394010948435794983e-01,2.320772854456423784e-01
CSIRO,1.579724395270813153e-01,0.000000000000000000e+00,8.938748433993150277e-02,6.615805708398354856e-02,4.992917021122253995e-01,9.396567422111294643e-02,4.516538676764009219e-01,9.454939227733365203e-02
DARSim,1.940029980493869766e-01,8.938748433993150277e-02,0.000000000000000000e+00,1.171796195443952776e-01,4.601948064421348961e-01,9.462792576606608719e-02,4.920340625966832526e-01,1.127097302576738347e-01
DARTS,1.460833131822168451e-01,6.615805708398354856e-02,1.171796195443952776e-01,0.000000000000000000e+00,5.077528851931735199e-01,1.132070587301931136e-01,4.434785592145091271e-01,1.118383111504548943e-01
LANL,6.468212986499282113e-01,4.992917021122253995e-01,4.601948064421348961e-01,5.077528851931735199e-01,0.000000000000000000e+00,4.580713751813252355e-01,9.491719948473569257e-01,4.195535259277853868e-01
Melbourne,2.016112504502489133e-01,9.396567422111294643e-02,9.462792576606608719e-02,1.132070587301931136e-01,4.580713751813252355e-01,0.000000000000000000e+00,4.924155351839590300e-01,1.358659581204569589e-01
Stanford,3.394010948435794983e-01,4.516538676764009219e-01,4.920340625966832526e-01,4.434785592145091271e-01,9.491719948473569257e-01,4.924155351839590300e-01,0.000000000000000000e+00,5.346784928421083327e-01
Stuttgart,2.320772854456423784e-01,9.454939227733365203e-02,1.127097302576738347e-01,1.118383111504548943e-01,4.195535259277853868e-01,1.358659581204569589e-01,5.346784928421083327e-01,0.000000000000000000e+00


==> distances/distances_72h.tex <==
distances, Austin, CSIRO, DARSim, DARTS, LANL, Melbourne, Stanford, Stuttgart
Austin,0.000000000000000000e+00,1.149174303212238540e-01,1.587726871403541962e-01,1.433635794625036375e-01,6.334438736769310019e-01,1.408314382379332041e-01,3.221744184981292225e-01,2.398062000606562272e-01
CSIRO,1.149174303212238540e-01,0.000000000000000000e+00,1.317942826964318415e-01,8.684634567065326050e-02,5.638595493070924780e-01,7.480008228737772269e-02,3.599256586934219126e-01,1.697558425590601772e-01
DARSim,1.587726871403541962e-01,1.317942826964318415e-01,0.000000000000000000e+00,1.317955718150244926e-01,4.831069016290849838e-01,9.887811916645908306e-02,4.368852409648979473e-01,1.462320894715338493e-01
DARTS,1.433635794625036375e-01,8.684634567065326050e-02,1.317955718150244926e-01,0.000000000000000000e+00,5.064671136687315389e-01,8.393906801930683947e-02,4.136960840141550300e-01,1.213695756282694715e-01
LANL,6.334438736769310019e-01,5.638595493070924780e-01,4.831069016290849838e-01,5.064671136687315389e-01,0.000000000000000000e+00,5.276146911997920963e-01,9.186845927210129936e-01,3.968058721145547030e-01
Melbourne,1.408314382379332041e-01,7.480008228737772269e-02,9.887811916645908306e-02,8.393906801930683947e-02,5.276146911997920963e-01,0.000000000000000000e+00,3.918454576696633884e-01,1.641981189890543147e-01
Stanford,3.221744184981292225e-01,3.599256586934219126e-01,4.368852409648979473e-01,4.136960840141550300e-01,9.186845927210129936e-01,3.918454576696633884e-01,0.000000000000000000e+00,5.255154392335171787e-01
Stuttgart,2.398062000606562272e-01,1.697558425590601772e-01,1.462320894715338493e-01,1.213695756282694715e-01,3.968058721145547030e-01,1.641981189890543147e-01,5.255154392335171787e-01,0.000000000000000000e+00


==> distances/distances_96h.tex <==
distances, Austin, CSIRO, DARSim, DARTS, LANL, Melbourne, Stanford, Stuttgart
Austin,0.000000000000000000e+00,1.081956818548097110e-01,1.371924705272896394e-01,1.334468278720781775e-01,6.135688839292939845e-01,1.101765363103290180e-01,3.119864355053298954e-01,2.280467324774274884e-01
CSIRO,1.081956818548097110e-01,0.000000000000000000e+00,1.589556745101045609e-01,9.810110621327190750e-02,6.103671999382546121e-01,6.814041768851540615e-02,3.334755122876750799e-01,2.245126579591803784e-01
DARSim,1.371924705272896394e-01,1.589556745101045609e-01,0.000000000000000000e+00,1.454949908892701760e-01,4.864069781656776836e-01,1.146592725123843082e-01,4.003232325835194283e-01,1.502355390132001367e-01
DARTS,1.334468278720781775e-01,9.810110621327190750e-02,1.454949908892701760e-01,0.000000000000000000e+00,5.267472570039529733e-01,7.384062881197778205e-02,3.608337056201051385e-01,1.426983325691176530e-01
LANL,6.135688839292939845e-01,6.103671999382546121e-01,4.864069781656776836e-01,5.267472570039529733e-01,0.000000000000000000e+00,5.744453015291312026e-01,8.857796497658974033e-01,3.873752463078847241e-01
Melbourne,1.101765363103290180e-01,6.814041768851540615e-02,1.146592725123843082e-01,7.384062881197778205e-02,5.744453015291312026e-01,0.000000000000000000e+00,3.144666521607527576e-01,1.957568926286935296e-01
Stanford,3.119864355053298954e-01,3.334755122876750799e-01,4.003232325835194283e-01,3.608337056201051385e-01,8.857796497658974033e-01,3.144666521607527576e-01,0.000000000000000000e+00,5.009781769516544747e-01
Stuttgart,2.280467324774274884e-01,2.245126579591803784e-01,1.502355390132001367e-01,1.426983325691176530e-01,3.873752463078847241e-01,1.957568926286935296e-01,5.009781769516544747e-01,0.000000000000000000e+00


==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}



==> sparse_data/austin.tex <==
idx,p10_mean,p50_mean,p90_mean,p10_dev,p50_dev,p90_dev
1a [N/m$^2$],111448.8311728,111486.7523528,112960.6107242,920.615104022203,907.914354190899,1466.23219142009
1b [N/m$^2$],105447.080488,105490.2072118,106343.9508688,433.555782215953,413.533747503411,775.213265491324
2 [s],18600,18600,18600,0,0,0
3a [kg],0.00170498521944805,0.00181943126883053,0.00210987610136608,0.00020786996148203,0.000148535275705598,0.000293245925109918
3b [kg],0.000295837675955342,0.000315298738951949,0.000345241731864876,2.96101590329268e-05,2.04093521021527e-05,3.44637186458377e-05
3c [kg],0.00115141630959182,0.00151292977138066,0.00198666554352747,0.000472465912296314,0.000296239812953546,0.000553107231052641
3d [kg],8.36964379052006e-05,0.000135819163802201,0.000330924268202632,0.000134793886279262,0.000111806574070829,0.000198789301357645
4a [kg],0,0,0,0,0,0
4b [kg],0,0,0,0,0,0
4c [kg],1.1998918962578e-06,4.4448600822998e-05,0.000251115599519648,0.00013912687134169,0.000121266868852786,0.000210075239875023
4d [kg],1.55858485334715e-12,7.85107343178575e-08,6.50487351240313e-06,3.32151664955502e-06,3.29032513502151e-06,5.97893720687521e-06
5 [s],13500,16200,18000,2830.19433961698,1632.17646104825,2683.28157299975
6 [kg],8.49190574418665e-05,0.000158140955011229,0.000337165025521797,0.000141698039508178,0.000108802394192001,0.000191960252017714


==> sparse_data/csiro.tex <==
idx, p10_mean, p50_mean, p90_mean, p10_dev, p50_dev, p90_dev
1a [N/m$^2$], 1.11415e5 , 1.11421e5 , 1.11431e5, 6.099 , 8.324 , 10.549
1b [N/m$^2$], 1.05513e5 , 1.05518e5 , 1.05524e5,  3.5283 , 5.7530 , 7.9778
2 [s], 1.800e4, 1.800e4,  1.800e4, 0, 0, 0
3a [kg], 1.665e-4, 3.487e-4, 8.331e-4, 2.894e-4, 3.901e-4, 4.909e-4
3b [kg], 0.0, 2.801e-7, 1.107e-5, 3.971e-6, 5.353e-6, 6.735e-6
3c [kg], 2.951e-3, 3.602e-3, 4.080e-3, 4.106e-4, 5.535e-4, 6.965e-4
3d [kg], 5.324e-4, 5.694e-4, 6.057e-4, 2.227e-5, 3.039e-5, 3.852e-5
4a [kg], 0.0, 0.0, 0.0, 0, 0, 0
4b [kg], 0.0, 0.0, 0.0, 0, 0, 0
4c [kg], 1.420e-4, 2.980e-4, 5.422e-4, 1.460e-4, 1.968e-4, 2.476e-4
4d [kg], 2.815e-7, 1.032e-7, 3.428e-7, 9.783e-7, 1.335e-6, 1.692e-6
5 [s], 6.109e4, 8.333e4, 1.281e5, 2.607e4, 3.515e4, 4.422e4
6 [kg], 5.332e-4, 5.724e-4, 6.611e-4, 5.381e-5, 7.344e-5, 9.307e-5


==> sparse_data/delft-darsim.tex <==
idx, p10_mean, p50_mean, p90_mean, p10_dev, p50_dev, p90_dev
1a [N/m$^2$],1.10E+05,1.10E+05,1.10E+05,1.92E+00,1.92E+00,1.92E+00
1b [N/m$^2$],1.04E+05,1.04E+05,1.04E+05,3.90E+00,3.90E+00,3.90E+00
2 [s],1.38E+04,1.41E+04,1.74E+04,1.68E+03,1.68E+03,1.68E+03
3a [kg],0.00E+00,7.61E-04,1.71E-03,7.12E-04,7.12E-04,7.12E-04
3b [kg],0.00E+00,0.00E+00,1.44E-05,7.85E-06,7.85E-06,7.85E-06
3c [kg],1.12E-03,2.20E-03,3.29E-03,9.06E-04,9.06E-04,9.06E-04
3d [kg],3.88E-06,6.68E-06,1.84E-05,6.59E-06,6.59E-06,6.59E-06
4a [kg],8.05E-10,2.43E-09,1.31E-05,6.67E-06,6.67E-06,6.67E-06
4b [kg],0.00E+00,0.00E+00,0.00E+00,0.00E+00,0.00E+00,0.00E+00
4c [kg],4.29E-04,6.26E-04,8.37E-04,1.80E-04,1.80E-04,1.80E-04
4d [kg],3.38E-09,1.33E-08,1.44E-07,7.46E-08,7.46E-08,7.46E-08
5 [s],n/a,n/a,n/a,n/a,n/a,n/a
6 [kg],6.68E-06,1.20E-05,2.65E-05,8.92E-06,8.92E-06,8.92E-06


==> sparse_data/delft-darts.tex <==
idx, p10_mean, p50_mean, p90_mean, p10_dev, p50_dev, p90_dev
1a [N/m$^2$],111092.907599,111182.346159,111243.951762,54.525473,54.525473,54.525473
1b [N/m$^2$],105235.791491,105299.623991,105342.052831,39.112776,39.112776,39.112776
2 [s],16200.000000,17400.000000,18000.000000,663.567295,663.567295,663.567295
3a [kg],0.000229,0.001145,0.001934,0.000627,0.000627,0.000627
3b [kg],0.000019,0.000083,0.000140,0.000044,0.000044,0.000044
3c [kg],0.001376,0.002318,0.003550,0.000802,0.000802,0.000802
3d [kg],0.000129,0.000398,0.000657,0.000213,0.000213,0.000213
4a [kg],0.000000,0.000000,0.000000,0.000001,0.000001,0.000001
4b [kg],0.000000,0.000000,0.000000,0.000000,0.000000,0.000000
4c [kg],0.000001,0.000010,0.000046,0.000029,0.000029,0.000029
4d [kg],0.000000,0.000000,0.000000,0.000001,0.000001,0.000001
5 [s],0.000000,0.000000,0.000000,0.000000,0.000000,0.000000
6 [kg],0.000214,0.000520,0.000658,0.000175,0.000175,0.000175


==> sparse_data/heriot-watt.tex <==
idx, p10_mean, p50_mean, p90_mean, p10_dev, p50_dev, p90_dev
1a [N/m$^2$], 109800, 109840, 109900, 20, 20, 20
1b [N/m$^2$], 103900, 103965, 104000, 20, 20, 20
2 [s], 18e3, 18.6e3, 19e3, 6e2, 6e2, 6e2
3a [kg], 0, 1e-3, 1.8e-3, 5e-4, 5e-4, 5e-4
3b [kg], 0, 1e-4, 3e-4, 1e-4, 1e-4, 1e-4
3c [kg], 1e-3, 2e-3, 4e-3, 1e-3, 1e-3, 1e-3
3d [kg], 0, 5e-4,9e-4, 3e-4, 3e-4, 3e-4
4a [kg], 0, 1e-5, 1e-4, 5e-7, 5e-6, 5e-5
4b [kg], 0, 1e-6, 1e-5, 5e-8, 5e-7, 5e-6
4c [kg], 0, 1e-4, 1e-3, 5e-5, 5e-5, 5e-4
4d [kg], 0, 2e-5, 1e-4, 5e-6, 5e-6, 5e-6
5 [s], 6e3, 10e3, 15e3, 1e3, 1e3, 1e3
6 [kg], 0, 5e-5, 1e-4, 0, 1e-5, 1e-4

==> sparse_data/lanl.tex <==
idx,p10_mean,p50_mean,p90_mean,p10_dev,p50_dev,p90_dev
1a [N/m$^2$],1.11E+05,1.11E+05,1.11E+05,1.00E+00,1.00E+00,1.00E+00
1b [N/m$^2$],1.05E+05,1.05E+05,1.05E+05,1.00E+00,1.00E+00,1.00E+00
2 [s],1.00E+11,1.00E+09,432000,432000,432000,432000
3a [kg],0.00E+00,0,0,1.00E-06,5.00E-07,1.00E-07
3b [kg],0.00E+00,0,0,1.00E-06,5.00E-07,1.00E-07
3c [kg],7.24E-05,7.24E-05,7.24E-05,1.00E-06,1.00E-06,1.00E-06
3d [kg],5.24E-05,5.24E-05,5.24E-05,1.00E-06,1.00E-06,1.00E-06
4a [kg],0.00E+00,0.00E+00,0.00E+00,1.00E-06,1.00E-06,1.00E-06
4b [kg],2.37E-05,2.37E-05,2.37E-05,1.00E-06,1.00E-06,1.00E-06
4c [kg],1.99E-03,1.99E-03,1.99E-03,1.00E-04,1.00E-04,1.00E-04
4d [kg],5.77E-04,5.77E-04,5.77E-04,1.00E-05,1.00E-05,1.00E-05
5 [s],8640000,8640000,8640000,3600,3600,3600
6 [kg],1.16E-04,1.16E-04,1.16E-04,1.00E-05,1.00E-05,1.00E-05

==> sparse_data/melbourne.tex <==
idx, p10_mean, p50_mean, p90_mean, p10_dev, p50_dev, p90_dev
1a [N/m$^2$],111709.5425,112375.7389,112880.9439,354.7457059,275.1280796,306.4205336
1b [N/m$^2$],104734.0265,105222.6039,105793.7958,236.0989309,187.6438417,278.6977969
2 [s],15984.17306,17092.6207,17897.94533,74.06407937,322.9962789,119.6955934
3a [kg],0.000402328,0.000582971,0.000750302,1.83E-05,3.84E-05,6.04E-05
3b [kg],n/a,n/a,n/a,n/a,n/a,n/a
3c [kg],0.003644835,0.003884338,0.004278152,n/a,n/a,n/a
3d [kg],0.000666583,0.000757962,0.000857116,0.000667221,0.000757962,0.000853543
4a [kg],3.16E-17,3.39E-17,3.81E-17,n/a,n/a,n/a
4b [kg],n/a,n/a,n/a,n/a,n/a,n/a
4c [kg],0.001570273,0.001611407,0.001619606,n/a,n/a,n/a
4d [kg],2.58E-06,3.81E-06,2.34E-05,n/a,n/a,n/a
5 [s],12283.62313,13059.20026,14023.2197,125.9389721,152.9597649,268.419846
6 [kg],n/a,n/a,n/a,n/a,n/a,n/a


==> sparse_data/stanford.tex <==
idx, p10_mean, p50_mean, p90_mean, p10_dev, p50_dev, p90_dev
1a [N/m$^2$], 1.111e+05, 1.113e+05, 1.115e+05, n/a, 2.369e+01, n/a
1b [N/m$^2$], 1.052e+05, 1.057e+05, 1.058e+05, n/a, 2.377e+01, n/a
2 [s], 1.820e+04, 2.664e+04, 2.314e+04, n/a, 1.834e+03, n/a
3a [kg], 0.000e+00, 1.895e-03, 2.259e-03, n/a, 8.569e-04, n/a
3b [kg], 1.955e-04, 2.033e-03, 5.894e-03, n/a, 2.931e-03, n/a
3c [kg], 1.218e-03, 5.288e-03, 5.642e-03, n/a, 2.060e-03, n/a
3d [kg], 1.365e-03, 2.040e-03, 5.987e-03, n/a, 2.702e-03, n/a
4a [kg], 0.000e+00, 0.000e+00, 2.231e-04, n/a, 1.663e-04, n/a
4b [kg], 0.000e+00, 0.000e+00, 2.697e-05, n/a, 2.010e-05, n/a
4c [kg], 7.800e-06, 4.502e-05, 2.147e-04, n/a, 9.521e-05, n/a
4d [kg], 0.000e+00, 0.000e+00, 0.000e+00, n/a, 0.000e+00, n/a
5 [s], 	  n/a, 1.350e+04, 	n/a, n/a, 	n/a, n/a
6 [kg], 1.362e-03, 2.033e-03, 5.982e-03, n/a, 2.703e-03, n/a


==> sparse_data/stuttgart.tex <==
idx,p10_mean,p50_mean,p90_mean,p10_dev,p50_dev,p90_dev
1a [N/m$^2$],n/a,109880.0,n/a,n/a,8.096638534327413,n/a
1b [N/m$^2$],n/a,103970.22222222222,n/a,n/a,6.214280646270917,n/a
2 [s],n/a,17666.666666666668,n/a,n/a,942.8090415820633,n/a
3a [kg],n/a,0.0019999674444444444,n/a,n/a,0.0005423896246211678,n/a
3b [kg],n/a,1.0066955555555557e-06,n/a,n/a,1.4252618568850281e-06,n/a
3c [kg],n/a,0.001600681111111111,n/a,n/a,0.0004961251058272488,n/a
3d [kg],n/a,0.00032009401111111115,n/a,n/a,0.0003485946279060487,n/a
4a [kg],n/a,1.7895e-06,n/a,n/a,4.061360060647446e-06,n/a
4b [kg],n/a,0.0,n/a,n/a,0.0,n/a
4c [kg],n/a,0.00039499966666666663,n/a,n/a,0.00025518252571792173,n/a
4d [kg],n/a,9.051329561555556e-06,n/a,n/a,1.2325226707772248e-05,n/a
5 [s],n/a,33933.333333333336,n/a,n/a,13798.872739788889,n/a
6 [kg],n/a,0.0003571286,n/a,n/a,0.0003926376724052851,n/a

